Monocular Depth Estimation using Diffusion Models

We formulate monocular depth estimation using denoising diffusion models, inspired by their recent successes in high fidelity image generation. To that end, we introduce innovations to address problems arising due to noisy, incomplete depth maps in training data, including step-unrolled denoising diffusion, an $L_1$ loss, and depth infilling during training. To cope with the limited availability of data for supervised training, we leverage pre-training on self-supervised image-to-image translation tasks. Despite the simplicity of the approach, with a generic loss and architecture, our DepthGen model achieves SOTA performance on the indoor NYU dataset, and near SOTA results on the outdoor KITTI dataset. Further, with a multimodal posterior, DepthGen naturally represents depth ambiguity (e.g., from transparent surfaces), and its zero-shot performance combined with depth imputation, enable a simple but effective text-to-3D pipeline. Project page: https://depth-gen.github.io

==> diffusion.tex <==
% \section{Background on diffusion}
% \label{diffusion}

\paragraph{Diffusion training and inference} Conditional diffusion models are trained to approximate a target distribution $p(\vy \mid \vx)$. For monocular depth estimation, $\vx$ is a RGB image and $\vy$ is the corresponding depth map.
In brief, a neural network $f_\theta$ is trained to predict the gradient of the log data distribution $\nabla_{y}\log p(\vy \mid \vx)$ (aka score), from which one can denoise a noisy signal $\vyt$ to estimate the noise-free signal.
The objective can be expressed as 
\begin{equation}
    \E_{(\vx,\, \vy)}\, \E_{(t,\, \veps)} \bigg\lVert f_\theta(\vx,\, \underbrace{\sqrt{\gamma_t} \,\vy + \sqrt{1\!-\!\gamma_t}\, \veps}_{\vyt}, \,t) - \veps\, \bigg\rVert^{p}_p
\label{eq:diffusion-loss}
\end{equation}
\begin{equation*}
    \veps \sim \mathcal{N}(0, I), \,t \sim \mathcal{U}(0, 1)
\end{equation*}
where ${\gamma_t}$ is computed with a pre-determined noise schedule.

Given the neural network to predict the score function $\nabla_{y}\log p(\vy \mid \vx)$, at inference time, one can draw samples from the data distribution $p(\vy \mid \vx)$ iteratively using \textit{Langevin dynamics}. In practice, one first draws a sample of Gaussian noise, and then iteratively applies the denoising network to incrementally remove noise, according to a sampler schedule, providing a fair sample from the target distribution upon completion.

Both $L_1$ \cite{saharia2021image} and $L_2$ \cite{ho2020denoising,sahariac-palette} losses have been used when training the denoising network on image to image translation problems. In Palette \cite{sahariac-palette}, they find an $L_1$ loss gives somewhat higher quality images, while $L_2$ tends to produce greater sample diversity.
Here, for RGB to depth map translation, our early empirical results suggested that an $L_1$ loss is more effective, likely because $L_1$ is somewhat robust to noise in training data, especially at larger depths.


==> multimodality_samples_old.tex <==
\def\kittiwidth{0.32}
\def\nyuwidth{0.24}
\def\boxcolor{lightgray}
\begin{figure*}
\begin{tabular}{cccc}
     &  Prediction 1 &  Prediction 2 & Groundtruth \\
    \includegraphics[width=\nyuwidth\textwidth]{figures/multimodality/living/rgb.png}
    &
    \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/living/depth1.png}
    &
    \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/living/depth2.png}
    &
    \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/living/gt.png}
    \\
    \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen/rgb.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen/depth4.png}& \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen/depth1.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen/gt.png} \\
    \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bed/rgb.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bed/depth1.png}& \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bed/depth2.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bed/gt.png} \\
    \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen1/rgb.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen1/depth1.png}& \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen1/depth3.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/kitchen1/gt.png} \\
    \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bath/rgb.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bath/depth1.png}& \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bath/depth2.png} & \includegraphics[width=\nyuwidth\linewidth]{figures/multimodality/bath/gt.png} \\
\end{tabular}
\caption{Multimodal depth predictions on the NYU Depth V2 val dataset. Rows 1-3 contain see-through doors/windows where the model learns to predict the depth for either the glass surface or the surface behind it. Row 4 has a dark door next to the refrigerator where it is unclear from the RGB image whether the door is open or closed. In row 5 the model hallucinates the reflected door as a cabinet, which seems plausible from the RGB image. \Abhishek{highlight  areas that differ across the two predictions (e.g. the transparent door in the row 1.}}

\vspace*{0.4cm}
\begin{tabular}{ccc}
     &  Prediction 1 &  Prediction 2 \\
    % \includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti1/rgb.png} & \includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti1/pred1.png}& \includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti1/pred2_labelled.png} \\
    % \includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti2/rgb.png}
    \begin{tikzpicture}[baseline={(current bounding box.south)}]
    \node[inner sep=0] at (0, 0) {\includegraphics[width=\kittiwidth\textwidth]{figures/multimodality/kitti2/rgb.png}};
    \draw[\boxcolor,ultra thin,dashed] (2.1,-0.1) rectangle (2.4, -0.5);
    \end{tikzpicture}
    & 
    \begin{tikzpicture}[baseline={(current bounding box.south)}]
    \node[inner sep=0] at (0, 0) {\includegraphics[width=\kittiwidth\textwidth]{figures/multimodality/kitti2/pred1.png}};
    \draw[\boxcolor,ultra thin,dashed] (2.1,-0.1) rectangle (2.4, -0.5);
    \end{tikzpicture}
    %\includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti2/pred1.png}
    & 
    \begin{tikzpicture}[baseline={(current bounding box.south)},spy using outlines={rectangle,\boxcolor,dashed,magnification=3,connect spies}]
    \node[inner sep=0] at (0, 0) {\includegraphics[width=\kittiwidth\textwidth]{figures/multimodality/kitti2/pred2.png}};
    \draw[\boxcolor,ultra thin,dashed] (2.1,-0.1) rectangle (2.4, -0.5);
    % \spy[width=1cm,height=1.2cm] on (2.25,-0.3) in node at (3.35,0.15);
    \end{tikzpicture}
    % \includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti2/pred2_labelled.png} 
    \\
    % \includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti1/rgb.png} 
    \begin{tikzpicture}[baseline={(current bounding box.south)}]
    \node[inner sep=0] at (0, 0) {\includegraphics[width=\kittiwidth\textwidth]{figures/multimodality/kitti1/rgb.png}};
    \draw[\boxcolor,ultra thin,dashed] (2.22,-0.1) rectangle (2.55, -0.4);
    \end{tikzpicture}
    & 
    \begin{tikzpicture}[baseline={(current bounding box.south)}]
    \node[inner sep=0] at (0, 0) {\includegraphics[width=\kittiwidth\textwidth]{figures/multimodality/kitti1/pred1.png}};
    \draw[\boxcolor,ultra thin,dashed] (2.22,-0.1) rectangle (2.55, -0.4);
    \end{tikzpicture}
    % \includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti1/pred1.png}
    & 
    \begin{tikzpicture}[baseline={(current bounding box.south)},spy using outlines={rectangle,\boxcolor,dashed,magnification=3,connect spies}]
    % [spy using outlines={rectangle, magnification=3,connect spies}] 

    \node[inner sep=0] at (0, 0) {\includegraphics[width=\kittiwidth\textwidth]{figures/multimodality/kitti1/pred2.png}};
    \draw[\boxcolor,ultra thin,dashed] (2.22,-0.1) rectangle (2.55, -0.4);
    % \spy[width=1cm,height=1cm] on (2.38,-0.25) in node at (3.35,0.3);
    \end{tikzpicture}

    %\includegraphics[width=\kittiwidth\linewidth]{figures/multimodality/kitti1/pred2_labelled.png}
\end{tabular}
\caption{Multimodal depth predictions on the KITTI val dataset. (GT depth has been omitted for readability.)}
\label{fig:multimodal_samples}
\end{figure*}

==> oldintro.tex <==
\section{Introduction [a new intro is WIP]}
\label{introduction}

Generative diffusion models are emerging as a powerful vehicle for high fidelity image generation, capturing what appears to be a remarkably high degree of knowledge about the visual world.
In addition to their ability to generate rich media for different uses cases, they also have remarkable potential 
% for the generation of synthetic training data (eg datasetGAN) and 
as pre-trained models for myriad downstream tasks. 
In this paper we explore the use of diffusion models for a well studied image-to-image translation task, namely, monocular depth estimation.
% We introduce \textit{\ours}, a model for high fidelity multi-modal monocular depth estimation.
% , leveraging self-supervised pre-trained models.

Pre-training is particularly useful for vision tasks where large scale 
training datasets are not available.
Here, we use a self-supervised pre-trained multi-task model that is trained using a combination of colorization, inpainting, uncropping and jpeg decompression. The pre-trained model is further trained with supervised depth on existing large-scale RGBD datasets, after which it can be fine-tuned to specific benchmarks or used zero-shot. Through careful ablations we show that unsupervised pretraining in this fashion substantially benefits the downstream depth estimation task. We showcase our model's robustness to out-of-distribution data by applying it to outputs of a text-to-image model Imagen.

Diffusion models have traditionally been trained to model well-behaved data distributions. Depth data on the other hand is sparse and has holes. This makes it challenging to model depth using iterative refinement. We propose several innovations to tackle this which may be more generally applicable to other tasks.

Unlike conventional regression models,  diffusion models provide the opportunity to sample from the posterior predictive distribution and do not suffer from mode collapse. We exploit the ability of diffusion models to accurately capture the multi-modal nature of the predictive distribution over depth given a single RGB image to uncover ambiguities in depth prediction. The iterative nature of these models also allows for zero-shot depth completion. We leverage this to build a pipeline for novel view synthesis, using existing image completion models, that supports moderate variations in camera pose.

% (Unlike some recent methods we do not rely on existing models like DPT to  generate depth for learning.)

% How well do SSL diffusion models perform as pre-trained models for subsequent fine-tuning or supervised refinement?

Compared to other methods with task-specific architectures and loss functions, our approach is both simple and generic.
The resulting model provides state-of-the-art results on conventional depth estimation benchmarks, generates high fidelity multi-modal depth maps with accurate object boundaries and provides zero-shot depth completion capabilities.
% It also provides a way to expand the scene through a combination of uncropping etc.

Our contributions are as follows:
\begin{enumerate}

\itemsep 0.1cm
\item We introduce a diffusion model for monocular depth estimation.
It leverages a self-supervised pre-trained model, with supervised fine-tuning, to achieve state-of-the-art relative error of \textit{0.074} on the challenging NYU dataset, without the need for specialized loss functions or neural architectures.
\item To enable training diffusion models with noisy, incomplete depth data, we advocate the use of a simple infilling technique and unbiased conditioning to reduce latent distribution shift between training and inference.
\item The probabilistic model is also shown to facilitate multimodal depth inference, and support zero-shot depth completion enabling a simple depth-aware approach to novel view synthesis.
\end{enumerate}

% \begin{enumerate}
% \item We show that self-supervised diffusion models can be fine-tuned for depth estimation, yielding SOTA performance on challenging benchmarks, without the need for specialized loss functions or neural architectures.
% \item To enable training diffusion models with noisy, incomplete depth data, we advocate the use of a simple infilling technique and unbiased conditioning to reduce latent distribution shift between training and inference.
% \item We show that the multimodal nature of diffusion models captures uncertainities in depth and iterative refinement enables zero-shot depth completion thereby
% providing a simple depth-aware approach to novel view
% synthesis.
% % Our depth diffusion model captures uncertainty allowing multi-modal predictive distributions, and they facilitate effective zero-shot depth completion with pose changes, supporting a simple depth-aware approach to novel view synthesis.
% \end{enumerate}

\begin{figure*}[t]
    \centering
    \begin{subfigure}
      \centering
      \includegraphics[width=\linewidth]{figures/architecture.pdf}
    \end{subfigure}
    \vspace*{-0.65cm}
    \caption{\label{fig:arch} Training Architecture}
\end{figure*}

